E$^3$-UAV: An Edge-based Energy-Efficient Object Detection System for Unmanned Aerial Vehicles

Motivated by the advances in deep learning techniques, the application of Unmanned Aerial Vehicle (UAV)-based object detection has proliferated across a range of fields, including vehicle counting, fire detection, and city monitoring. While most existing research studies only a subset of the challenges inherent to UAV-based object detection, there are few studies that balance various aspects to design a practical system for energy consumption reduction. In response, we present the E$^3$-UAV, an edge-based energy-efficient object detection system for UAVs. The system is designed to dynamically support various UAV devices, edge devices, and detection algorithms, with the aim of minimizing energy consumption by deciding the most energy-efficient flight parameters (including flight altitude, flight speed, detection algorithm, and sampling rate) required to fulfill the detection requirements of the task. We first present an effective evaluation metric for actual tasks and construct a transparent energy consumption model based on hundreds of actual flight data to formalize the relationship between energy consumption and flight parameters. Then we present a lightweight energy-efficient priority decision algorithm based on a large quantity of actual flight data to assist the system in deciding flight parameters. Finally, we evaluate the performance of the system, and our experimental results demonstrate that it can significantly decrease energy consumption in real-world scenarios. Additionally, we provide four insights that can assist researchers and engineers in their efforts to study UAV-based object detection further.

==> 8_reference_bib.tex <==
\begin{thebibliography}{99}
% \bibliographystyle{IEEEtran}

\bibitem{vehicle_count} Amato, Giuseppe, et al. "Counting vehicles with deep learning in onboard uav imagery." 2019 IEEE Symposium on Computers and Communications (ISCC). IEEE, 2019.

\bibitem{fire_detection} Yuan, Chi, Zhixiang Liu, and Youmin Zhang. "UAV-based forest fire detection and tracking using image processing techniques." 2015 International Conference on Unmanned Aircraft Systems (ICUAS). IEEE, 2015.

\bibitem{city_monitoring} Puri, Anuj, K. P. Valavanis, and M. Kontitsis. "Statistical profile generation for traffic monitoring using real-time UAV based video data." 2007 Mediterranean Conference on Control \& Automation. IEEE, 2007.

\bibitem{rescue} Silvagni, Mario, et al. "Multipurpose UAV for search and rescue operations in mountain avalanche events." Geomatics, Natural Hazards and Risk 8.1 (2017): 18-33.

\bibitem{zhu2018vision} Zhu, Pengfei, et al. "Vision meets drones: A challenge." arXiv preprint arXiv:1804.07437 (2018).

\bibitem{standford} Robicquet, Alexandre, et al. "Learning social etiquette: Human trajectory understanding in crowded scenes." European conference on computer vision. Springer, Cham, 2016.

\bibitem{uav123} Mueller, Matthias, Neil Smith, and Bernard Ghanem. "A benchmark and simulator for uav tracking." European conference on computer vision. Springer, Cham, 2016.

\bibitem{CARPK} Hsieh, Meng-Ru, Yen-Liang Lin, and Winston H. Hsu. "Drone-based object counting by spatially regularized regional proposal network." Proceedings of the IEEE international conference on computer vision. 2017.

\bibitem{au-air} Bozcan, Ilker, and Erdal Kayacan. "Au-air: A multi-modal unmanned aerial vehicle dataset for low altitude traffic surveillance." 2020 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2020.

\bibitem{asl-tid} Portmann, Jan, et al. "People detection and tracking from aerial thermal views." 2014 IEEE international conference on robotics and automation (ICRA). IEEE, 2014.

\bibitem{BIRDSAI} Bondi, Elizabeth, et al. "BIRDSAI: A dataset for detection and tracking in aerial thermal infrared videos." Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision. 2020.

\bibitem{FLAME} Shamsoshoara, Alireza, et al. "Aerial imagery pile burn detection using deep learning: The FLAME dataset." Computer Networks 193 (2021): 108001.

\bibitem{algo_pre_1_rrnet} Chen, Changrui, et al. "Rrnet: A hybrid detector for object detection in drone-captured images." Proceedings of the IEEE/CVF International Conference on Computer Vision Workshops. 2019.

\bibitem{algo_pre_2_Towards} Yu, Weiping, Taojiannan Yang, and Chen Chen. "Towards resolving the challenge of long-tail distribution in UAV images for object detection." Proceedings of the IEEE/CVF winter conference on applications of computer vision. 2021.

\bibitem{algo_pre_3_roi} Ding, Jian, et al. "Learning RoI transformer for oriented object detection in aerial images." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2019.

\bibitem{algo_pre_4_TPH-YOLOv5} Zhu, Xingkui, et al. "TPH-YOLOv5: Improved YOLOv5 based on transformer prediction head for object detection on drone-captured scenarios." Proceedings of the IEEE/CVF International Conference on Computer Vision. 2021.

\bibitem{algo_pre_5_Uav-yolo} Liu, Mingjie, et al. "Uav-yolo: Small object detection on unmanned aerial vehicle perspective." Sensors 20.8 (2020): 2238.

\bibitem{algo_pre_6_SyNet} Albaba, Berat Mert, and Sedat Ozer. "SyNet: An ensemble network for object detection in UAV images." 2020 25th International Conference on Pattern Recognition (ICPR). IEEE, 2021.

\bibitem{algo_pre_7_zhang2019dense} Zhang, Xindi, Ebroul Izquierdo, and Krishna Chandramouli. "Dense and small object detection in uav vision based on cascade network." Proceedings of the IEEE/CVF International Conference on Computer Vision Workshops. 2019.

\bibitem{algo_energy_1_xu2019dac} Xu, Xiaowei, et al. "Dac-sdc low power object detection challenge for uav applications." IEEE transactions on pattern analysis and machine intelligence 43.2 (2019): 392-403.

\bibitem{algo_energy_2_deng2019energy} Deng, Jianing, Zhiguo Shi, and Cheng Zhuo. "Energy-efficient real-time UAV object detection on embedded platforms." IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems 39.10 (2019): 3123-3127.

\bibitem{algo_energy_3_zhang2019skynet} Zhang, Xiaofan, et al. "Skynet: A champion model for dac-sdc on low power object detection." arXiv preprint arXiv:1906.10327 (2019).

\bibitem{communication_1_zeng2019energy} Zeng, Yong, Jie Xu, and Rui Zhang. "Energy minimization for wireless communication with rotary-wing UAV." IEEE Transactions on Wireless Communications 18.4 (2019): 2329-2345.

\bibitem{communication_2_yang2019energy} Yang, Zhaohui, Wei Xu, and Mohammad Shikh-Bahaei. "Energy efficient UAV communication with energy harvesting." IEEE Transactions on Vehicular Technology 69.2 (2019): 1913-1927.

\bibitem{communication_3_zhou2018mobile} Zhou, Zhenyu, et al. "When mobile crowd sensing meets UAV: Energy-efficient task assignment and route planning." IEEE Transactions on Communications 66.11 (2018): 5526-5538.

\bibitem{communication_4_li2020energy} Li, Mushu, et al. "Energy-efficient UAV-assisted mobile edge computing: Resource allocation and trajectory optimization." IEEE Transactions on Vehicular Technology 69.3 (2020): 3424-3438.

\bibitem{communication_5_tran2020coarse} Tran, Dinh-Hieu, et al. "Coarse trajectory design for energy minimization in UAV-enabled." IEEE Transactions on Vehicular Technology 69.9 (2020): 9483-9496.

\bibitem{sys_1_tijtgat2017embedded} Tijtgat, Nils, et al. "Embedded real-time object detection for a UAV warning system." Proceedings of the IEEE international conference on computer vision workshops. 2017.

\bibitem{sys_2_boubin2019managing} Boubin, Jayson G., et al. "Managing edge resources for fully autonomous aerial systems." Proceedings of the 4th ACM/IEEE Symposium on Edge Computing. 2019.

\bibitem{sys_3_li2019intelligent} Li, Chuanlong, Xingming Sun, and Junhao Cai. "Intelligent mobile drone system based on real-time object detection." Journal of Artificial Intelligence 1.1 (2019): 1.

\bibitem{sys_5_madasamy2021osddy} Madasamy, Kaliappan, et al. "OSDDY: embedded system-based object surveillance detection system with small drone using deep YOLO." EURASIP Journal on Image and Video Processing 2021.1 (2021): 1-14.

\bibitem{sys_6_nguyen2021visual} Nguyen, A. Q., et al. "A visual real-time fire detection using single shot multibox detector for uav-based fire surveillance." 2020 IEEE Eighth International Conference on Communications and Electronics (ICCE). IEEE, 2021.

\bibitem{sys_7_lee2017real} Lee, Jangwon, et al. "Real-time, cloud-based object detection for unmanned aerial vehicles." 2017 First IEEE International Conference on Robotic Computing (IRC). IEEE, 2017.

\bibitem{visdrone2019} Zhu, Pengfei, et al. "Detection and tracking meet drones challenge." IEEE Transactions on Pattern Analysis and Machine Intelligence 44.11 (2021): 7380-7399.

\bibitem{lin2014microsoft} Lin, Tsung-Yi, et al. "Microsoft coco: Common objects in context." European conference on computer vision. Springer, Cham, 2014.

\bibitem{zhang2022dino} Zhang, Hao, et al. "Dino: Detr with improved denoising anchor boxes for end-to-end object detection." arXiv preprint arXiv:2203.03605 (2022).

\bibitem{rcnn} Girshick, Ross, et al. "Rich feature hierarchies for accurate object detection and semantic segmentation." Proceedings of the IEEE conference on computer vision and pattern recognition. 2014.

\bibitem{fastrcnn} Girshick, Ross. "Fast r-cnn." Proceedings of the IEEE international conference on computer vision. 2015.

\bibitem{fasterrcnn} Ren, Shaoqing, et al. "Faster r-cnn: Towards real-time object detection with region proposal networks." Advances in neural information processing systems 28 (2015).

\bibitem{yolov1} Redmon, Joseph, et al. "You only look once: Unified, real-time object detection." Proceedings of the IEEE conference on computer vision and pattern recognition. 2016.

\bibitem{yolov2} Redmon, Joseph, and Ali Farhadi. "YOLO9000: better, faster, stronger." Proceedings of the IEEE conference on computer vision and pattern recognition. 2017.

\bibitem{yolov3} Redmon, Joseph, and Ali Farhadi. "Yolov3: An incremental improvement." arXiv preprint arXiv:1804.02767 (2018).

\bibitem{yolov4} Bochkovskiy, Alexey, Chien-Yao Wang, and Hong-Yuan Mark Liao. "Yolov4: Optimal speed and accuracy of object detection." arXiv preprint arXiv:2004.10934 (2020).

\bibitem{ssd} Liu, Wei, et al. "Ssd: Single shot multibox detector." European conference on computer vision. Springer, Cham, 2016.

\bibitem{DOTA} Xia, Gui-Song, et al. "DOTA: A large-scale dataset for object detection in aerial images." Proceedings of the IEEE conference on computer vision and pattern recognition. 2018.

\bibitem{HRSC2016} Liu, Zikun, et al. "A high resolution optical satellite image dataset for ship recognition and some new baselines." International conference on pattern recognition applications and methods. Vol. 2. SciTePress, 2017.

\bibitem{algo_deployment_1_kyrkou2018dronet} Kyrkou, Christos, et al. "DroNet: Efficient convolutional neural network detector for real-time UAV applications." 2018 Design, Automation \& Test in Europe Conference \& Exhibition (DATE). IEEE, 2018.

\bibitem{algo_deployment_2_majid2018shuffledet} Majid Azimi, Seyed. "Shuffledet: real-time vehicle detection network in on-board embedded uav imagery." Proceedings of the European Conference on Computer Vision (ECCV) Workshops. 2018.

\bibitem{algo_deployment_3_balamuralidhar2021multeye} Balamuralidhar, Navaneeth, Sofia Tilon, and Francesco Nex. "MultEYE: Monitoring system for real-time vehicle detection, tracking and speed estimation from UAV imagery on edge-computing platforms." Remote sensing 13.4 (2021): 573.

\bibitem{algo_deployment_4_zhang2019slimyolov3} Zhang, Pengyi, Yunxin Zhong, and Xiaoqiong Li. "SlimYOLOv3: Narrower, faster and better for real-time UAV applications." Proceedings of the IEEE/CVF International Conference on Computer Vision Workshops. 2019.

\bibitem{suo2021feasibility} Suo, Jiashun, et al. "Feasibility Analysis of Machine Learning Optimization on GPU-based Low-cost Edges." 2021 IEEE SmartWorld, Ubiquitous Intelligence \& Computing, Advanced \& Trusted Computing, Scalable Computing \& Communications, Internet of People and Smart City Innovation (SmartWorld/SCALCOM/UIC/ATC/IOP/SCI). IEEE, 2021.

\end{thebibliography}
